Accurate and efficient approximation of large-scale appointment schedules

Setting up optimal appointment schedules requires the computation of an inherently involved objective function, typically requiring distributional knowledge of the clients' waiting times and the server's idle times (as a function of the appointment times of the individual clients). A frequently used idea is to approximate the clients' service times by their phase-type counterpart, thus leading to explicit expressions for the waiting-time and idle-time distributions. This method, however, requires the evaluation of the matrix exponential of potentially large matrices, which already becomes prohibitively slow from, say, 20 clients on. In this paper we remedy this issue by recursively approximating the distributions involved relying on a two-moments fit. More specifically, we approximate the sojourn time of each of the clients by a low-dimensional phase-type, Weibull or Lognormal random variable with the desired mean and variance. Our computational experiments show that this elementary, yet highly accurate, technique facilitates the evaluation of optimal appointment schedules even if the number of clients is large. The three ways to approximate the sojourn-time distribution turn out to be roughly equally accurate, except in certain specific regimes, where the low-dimensional phase-type fit performs well across all instances considered. As this low-dimensional phase-type fit is by far the fastest of the three alternatives, it is the approximation that we recommend.

==> Sections/algorithms-old.tex <==
\section{Algorithms}\label{ALG}

We now use the ideas presented in Section \ref{PREL} to develop our numerical technique to approximate the objective function ${\mathscr L}({\boldsymbol x})$, as defined in \eqref{OBJ}. The main idea is that we iteratively apply a two-moments phase-type fit, a Weibull fit, or a Lognormal fit to the sojourn-time distribution. 

\subsection{Fit of sojourn times} %In Section \ref{EOF} it was assumed that the sojourn times have a hyperexponential or mixed Erlang distribution, which is in general not true. 
In the present section we determine a phase-type fit (being either hyperexponential or mixed Erlang), Weibull fit, and Lognormal fit based on the respective distribution of sojourn time as mentioned in Section \ref{EOF}.

We start by reviewing a number of standard identities. For a non-negative continuous random variable $X$ and positive number $x$,
\[{\mathbb E}\,\max\{X-x,0\} = \int_{(0,\infty)} yf_X(y+x)\,{\rm d}y. \]
Along the same lines,
\[{\mathbb V}{\rm ar}\,\max\{X-x,0\} = \int_{(0,\infty)} y^2f_X(y+x)\,{\rm d}y-\left(\int_{(0,\infty)} yf_X(y+x)\,{\rm d}y\right)^2.\]
Applying the Lindley recursion \eqref{LR}, and recalling that $R_i$ and $B_{i+1}$ are independent, this immediately entails that
\begin{equation}\label{Ri}r_{i+1}:={\mathbb E}\,R_{i+1}= \int_{(0,\infty)} yf_{R_i}(y+x_i)\,{\rm d}y + \beta_{i+1},\end{equation}
and likewise
\begin{equation}\label{Vi}v_{i+1}:={\mathbb V}{\rm ar}\,R_{i+1}= \int_{(0,\infty)} y^2f_{R_i}(y+x_i)\,{\rm d}y-\left(\int_{(0,\infty)} yf_{R_i}(y+x_i)\,{\rm d}y\right)^2 +\sigma_{i+1}^2.\end{equation}
The next goal is to compute $r_{i+1}$ and $v_{i+1}$ for our phase-type fit, Weibull fit, and Lognormal fit. 

\subsubsection{Phase-type fit}
We proceed by evaluating \eqref{Ri} and \eqref{Vi} for the hyperexponential and mixed Erlang case, respectively. 
\begin{itemize}
    \item[$\circ$] 
Suppose $R_i\sim {\rm HE}(\alpha,\mu_1,\mu_2)$. As a direct application of \eqref{Ri}, we conclude that the mean of the $(i+1)$-st sojourn time is given by
\begin{align}\notag
    r_{i+1}&=\int_0^\infty y f_{R_i}(y+x_i) \,{\rm d}y +\beta_{i+1} = \int_0^\infty y\left(\alpha\mu_1 e^{-\mu_1(y+x_i)} 
    +(1-\alpha)\mu_2 e^{-\mu_2(y+x_i)}\right) {\rm d}y +\beta_{i+1} \\
    &= \frac{\alpha}{\mu_1} e^{-\mu_1 x_i}+\frac{1-\alpha}{\mu_2} e^{-\mu_2 x_i} +\beta_{i+1}.\label{RiHE}
\end{align}
Likewise, for the variance we find due to \eqref{Vi}, 
\begin{align}
    v_{i+1} & = 2\left(\frac{\alpha}{\mu_1^2} e^{-\mu_1 x_i}+\frac{1-\alpha}{\mu_2^2} e^{-\mu_2 x_i}\right) -\left( \frac{\alpha}{\mu_1} e^{-\mu_1 x_i}+\frac{1-\alpha}{\mu_2} e^{-\mu_2 x_i} \right)^2 +\sigma_{i+1}^2.\label{ViHE}
\end{align}

\item[$\circ$]  Suppose $R_i\sim {\rm ME}(p,k,\mu)$.  The computations for this case, with the corresponding density given by \eqref{MED},  are slightly more tedious. 
After a few steps of elementary calculus, involving a substitution, it follows that
\begin{align*}
\int_0^\infty y \mu^k (y+x)^{k-1} e^{-\mu (y+x)}\,{\rm d}y &=\frac{1}{\mu} \Gamma (k+1, \mu x) -x\, \Gamma(k, \mu x) \\
& = \Gamma(k, \mu x)\Big( \frac{k}{\mu}-x\Big)+ \mu^{k-1}x^k e^{-\mu x} =:M (k,x,\mu).
\end{align*}  Analogously, we find
that
\begin{align*}
\int_0^\infty y^2 \mu^k &(y+x)^{k-1} e^{-\mu (y+x)}\,{\rm d}y  =\frac{1}{\mu^2}\Gamma(k+2, \mu x) - \frac{2x}{\mu} \Gamma(k+1, \mu x)+ x^2 \Gamma(k, \mu x) \\
& = \Gamma(k+1,\mu x)\Big( \frac{k+1-2\mu x}{\mu^2}\Big)+x^2\Gamma(k, \mu x)+ \mu^{k-1}x^{k+1}e^{-\mu x} \\
& = \Gamma(k,\mu x)\frac{k+(k-\mu x)^2}{\mu^2} + e^{-\mu x}\mu^{k-2}x^k(k+1-\mu x)  =:S (k,x,\mu).
\end{align*}
We thus find, applying \eqref{Ri},
\begin{equation}\label{RiME}r_{i+1} = \frac{p}{(k-2)!}\,M (k-1,x_i,\mu)+\frac{1-p}{(k-1)!}\,M (k,x_i,\mu)+\beta_{i+1}
\end{equation}
and, by \eqref{Vi}, and with $r_{i+1}$ given by \eqref{RiME},
\begin{align}\notag v_{i+1}&=\frac{p}{(k-2)!}\,S (k-1,x_i,\mu)+\frac{1-p}{(k-1)!}\,S (k,x_i,\mu)\,-\\ \label{ViME}
&\:\:\:\left(\frac{p}{(k-2)!}\,M (k-1,x_i,\mu)+\frac{1-p}{(k-1)!}\,M (k,x_i,\mu)\right)^2+\sigma^2_{i+1}.\end{align}
\end{itemize}


%THE NEXT PART HAS BEEN COMMENTED OUT
\iffalse
For mean, (For K phases)
\begin{align*}
    \int_0^\infty x f_B(x+t) dx  & =\int_0^\infty \frac{x \mu^k (x+t)^{k-1} e^{-\mu (x+t)}}{(k-1)!} dx\\
    & = \frac{\mu^k}{(k-1)!} \int_t^\infty (u-t)u^{k-1}e^{-\mu u} du ~~~~\text{Set} ~x+t=u\\
    & = \frac{\mu^k}{(k-1)!} \Bigg[ \int_t^\infty u^k e^{-\mu u}du - t \int_t^\infty u^{k-1} e^{-\mu u}du \Bigg] \\
    & = \frac{1}{(k-1)!} \Bigg[ \int_t^\infty (\mu u)^k e^{-\mu u}du - t\mu \int_t^\infty (\mu u)^{k-1} e^{-\mu u}du \Bigg] \\
    & = \frac{1}{(k-1)!} \Bigg[ \frac{1}{\mu} \int_{\mu t}^\infty (z)^k e^{- z}dz - t\int_{\mu t}^\infty (z)^{k-1} e^{-z}dz  \Bigg]  ~~~~\text{Set}~\mu u =z \\
    & =  \frac{1}{(k-1)!}  \Bigg[ \frac{1}{\mu} \Gamma (k+1, \mu t) -t \Gamma(k, \mu t) \Bigg]
\end{align*}

\begin{align*}
     \int_0^\infty x^2 f_B(x+t) dx & = \int_0^\infty \frac{x^2 \mu^k (x+t)^{k-1} e^{-\mu (x+t)}}{(k-1)!} dx \\
     & = \frac{\mu^k}{(k-1)!} \int_t^\infty (u-t)^2 u^{k-1}e^{-\mu u} du ~~~~\text{Set} ~x+t=u\\
     & = \frac{1}{(k-1)!} \Bigg[ \int_t^\infty \frac{(u\mu)^{k+1} e^{-u\mu}}{\mu} du -2t \int_t^\infty (u\mu)^{k} e^{-u\mu} du + t^2 \mu\int_t^\infty (u\mu)^{k-1}e^{-u\mu} du \Bigg] \\
     & = \frac{1}{(k-1)!} \Bigg[ \int_{\mu t}^\infty \frac{(z)^{k+1} e^{-z}}{\mu^2} dz -\frac{2t}{\mu} \int_{\mu t}^\infty (z)^{k} e^{-z} dz + t^2 \int_{\mu t}^\infty (z)^{k-1}e^{-z} dz \Bigg]   ~~~~\text{Set}~\mu u =z \\
     & = \frac{1}{(k-1)!} \Bigg[ \frac{1}{\mu^2}\Gamma(k+2, \mu t) - \frac{2t}{\mu} \Gamma(k+1, \mu t)+ t^2 \Gamma(k, \mu t)  \Bigg]
\end{align*}

For variance
 \begin{align*}
    \mathbb{V}ar [max \{B-t, 0\}] & = \mathbb{E}[max \{B-t, 0\} ^2] - {\mathbb{E}[max \{B-t, 0\}]}^2 \\
    & =  \frac{1}{(k-1)!} \Bigg[ \frac{1}{\mu^2}\Gamma(k+2, \mu t) - \frac{2t}{\mu} \Gamma(k+1, \mu t)+ t^2 \Gamma(k, \mu t)  \Bigg] \\
    & - \Bigg\{ \frac{1}{(k-1)!}  \Bigg[ \frac{1}{\mu} \Gamma (k+1, \mu t) -t \Gamma(k, \mu t) \Bigg] \Bigg\}^2
 \end{align*}

 Mean (For K-1 phases): 

 \begin{align*}
    \int_0^\infty x f_B(x+t) dx  & =\int_0^\infty \frac{x \mu^{k-1} (x+t)^{k-2} e^{-\mu (x+t)}}{(k-2)!} dx\\
    & =  \frac{1}{(k-2)!}  \Bigg[ \frac{1}{\mu} \Gamma (k, \mu t) -t \Gamma(k-1, \mu t) \Bigg], ~~~~\text{following calculations like above}.
\end{align*}

\begin{align*}
    \int_0^\infty x^2 f_B(x+t) dx  & =\int_0^\infty \frac{x^2 \mu^{k-1} (x+t)^{k-2} e^{-\mu (x+t)}}{(k-2)!} dx\\
    & = \frac{1}{(k-2)!} \Bigg[ \frac{1}{\mu^2}\Gamma(k+1, \mu t) - \frac{2t}{\mu} \Gamma(k, \mu t)+ t^2 \Gamma(k-1, \mu t)  \Bigg]
\end{align*}

Finally, combining both $K$ and $K-1$ phases we get:

\begin{equation*}
  \text{Mean} =  \frac{p}{(k-2)!} \Bigg[ \frac{1}{\mu} \Gamma (k, \mu t) -t \Gamma(k-1, \mu t) \Bigg] +\frac{1-p)}{(k-1)!}  \Bigg[ \frac{1}{\mu} \Gamma (k+1, \mu t) -t \Gamma(k, \mu t) \Bigg] 
\end{equation*}

\begin{align*}
    \text{Variance} & =  \frac{p}{(k-2)!} \Bigg[ \frac{1}{\mu^2}\Gamma(k+1, \mu t) - \frac{2t}{\mu} \Gamma(k, \mu t)+ t^2 \Gamma(k-1, \mu t)  \Bigg] \\
    & - \Bigg\{ \frac{p}{(k-2)!}  \Bigg[ \frac{1}{\mu} \Gamma (k, \mu t) -t \Gamma(k-1, \mu t) \Bigg] \Bigg\}^2\\
    & +  \frac{(1-p)}{(k-1)!} \Bigg[ \frac{1}{\mu^2}\Gamma(k+2, \mu t) - \frac{2t}{\mu} \Gamma(k+1, \mu t)+ t^2 \Gamma(k, \mu t)  \Bigg] \\
    & - \Bigg\{ \frac{(1-p)}{(k-1)!}  \Bigg[ \frac{1}{\mu} \Gamma (k+1, \mu t) -t \Gamma(k, \mu t) \Bigg] \Bigg\}^2
\end{align*}
\fi 

\subsubsection{Weibull fit}
Now suppose that $R_i \sim {\rm W}(\lambda, \alpha)$.  Then a routine calculation yields
\begin{align} 
    r_{i+1} &= \int_0^\infty y f_{R_i}(y+x_i) \,{\rm d}y +\beta_{i+1}  = \frac{1}{\lambda} \Gamma (1+{1}/{\alpha}, (\lambda x)^\alpha) - x e^{-(\lambda x)^\alpha} + \beta_{i+1}.\label{RiW}
\end{align}
For the corresponding variance, we find, after a few intermediate steps, 
\begin{align}
 \notag   v_{i+1} & 
    %= \int_{(0,\infty)} y^2f_{R_i}(y+x_i)\,{\rm d}y-\left(\int_{(0,\infty)} yf_{R_i}( y+x_i)\,{\rm d}y\right)^2 +\sigma_{i+1}^2\notag \\ \notag
%    & =  \int_{(\lambda x)^\alpha}^\infty \Bigg( \frac{w^{\frac{1}{\alpha}}}{\lambda}-x\Bigg)^2e^{-w}dw - \left(\int_{(0,\infty)} yf_{R_i}( y+x_i)\,{\rm d}y\right)^2 +\sigma_{i+1}^2 \\ \notag & 
=\frac{1}{\lambda^2}\Gamma(1+{2}/{\alpha},(\lambda x)^\alpha) -\frac{2x}{\lambda}\Gamma(1+{1}/{\alpha}, (\lambda x)^\alpha) + x^2 e^{-(\lambda x)^\alpha} \:-\\ &\hspace{2cm}\left(\frac{1}{\lambda} \Gamma (1+{1}/{\alpha}, (\lambda x)^\alpha) - x e^{-(\lambda x)^\alpha} \right)^2 + \sigma_{i+1}^2.\label{ViW}
\end{align}

\subsubsection{Lognormal fit}
Finally, suppose that $R_i \sim {\rm LN}(\mu, \tau^2)$. Then,
\begin{equation}\label{RiLN} r_{i+1}  = e^{\mu+\tau^2/2} \,\Psi\left(\frac{\log x - \mu-\tau^2}{\tau}\right) - x \,\Psi\left(\frac{\log x-\mu }{\tau}\right) + \beta_{i+1} .\end{equation}
Also the variance can be computed using the same steps as before. We thus arrive at
\iffalse
\begin{align*}
    \int_{(0,\infty)} y^2f_{R_i}(y+x_i)\,{\rm d}y & =  \int_{(0,\infty)} \frac{y^2 e^{-\frac{(log(x+y)-\mu)^2}{2\tau^2}}dy}{\tau\sqrt{2\pi}(y+x)} \\
     & = \int_{logx}^{\infty}\frac{(e^w-x)^2 e^{-\frac{(w-\mu)^2dw}{2\tau^2}}}{\tau\sqrt{2\pi}}\\ & =  \int_{logx}^{\infty}e^{2w} \frac{ e^{-\frac{(w-\mu)^2dw}{2\tau^2}}}{\tau\sqrt{2\pi}} -2x  \int_{logx}^{\infty} e^{2w} \frac{ e^{-\frac{(w-\mu)^2dw}{2\tau^2}}}{\tau\sqrt{2\pi}} + x^2 \int_{logx}^{\infty}\frac{ e^{-\frac{(w-\mu)^2dw}{2\tau^2}}}{\tau\sqrt{2\pi}}\\
     & = \int_{logx}^{\infty}e^{2(\mu +\tau^2)} \frac{ e^{-\frac{(w-(\mu + 2\tau^2))^2}{2\tau^2}}}{\tau \sqrt{2\pi}} -2x\, e^{\mu+\tau^2/2} \Psi\left(\frac{\log x - \mu-\tau^2}{\tau}\right) + x^2\,\Psi\left(\frac{\log x-\mu}{\tau}\right) 
\end{align*}
where, last parts of this terms are calculated in \ref{ELN}, and using complete square in first part.
\fi
\begin{align}\notag
v_{i+1} &=  e^{2(\mu + \tau^2)}\Psi\left( \frac{\log x-\mu -2\tau^2}{\tau} \right) -2x\, e^{\mu+\tau^2/2} \Psi\left(\frac{\log x - \mu-\tau^2}{\tau}\right) +x^2\, \Psi \left(\frac{\log x-\mu }{\tau} \right) \:-\\
& \hspace{2cm} \left(e^{\mu+\tau^2/2} \,\Psi\left(\frac{\log x - \mu-\tau^2}{\tau}\right) - x \,\Psi\left(\frac{\log x-\mu}{\tau}\right)\right)^2 +\sigma_{i+1}^2 .\label{ViLN}
\end{align}

\subsection{Pseudocode of algorithm}
Using the ideas developed in Section \ref{PREL}, we are now in a position to describe our algorithm to approximate the objective function \eqref{OBJ}. The main idea is that for every client $i$ we approximate the mean $r_i$ and variance $v_i$ of her sojourn time, based on the mean $r_{i-1}$ and variance $v_{i-1}$ of the sojourn time of her predecessor, using the three fits introduced above.
The pseudocode for the resulting three approximation algorithms, that we display below, is self-explanatory. Observe that the complexity of each of the algorithms is $O(n)$.

\vspace{3mm}

{\small
\begin{algorithm}[H]
 \KwData{$(\beta_1,\ldots,\beta_n)$,  $(\sigma_1^2,\ldots,\sigma_n^2)$, $(x_1,\ldots,x_n)$.}
 \KwResult{$(r_1,\ldots,r_n)$,  $(v_1,\ldots,v_n),$ ${\mathscr L}^{({\rm Ph})} ( {\boldsymbol x})$.}
 Initialization: $i:=1$\;
 $r_1:=\beta_1$, $v_1:=\sigma_1^2$\;
  ${\mathscr L}^{({\rm Ph})} ( {\boldsymbol x}):=0$\;
 \While{$i < n$}{
  \eIf{$r_i^2\leqslant v_i$}{
   Perform HE phase-type fit: given $r_i$ and $v_i$, determine $\alpha,\mu_1,\mu_2$\;
   ${\mathscr L}^{({\rm Ph})} ( {\boldsymbol x}):={\mathscr L}^{({\rm Ph})} ( {\boldsymbol x})+{\mathscr L}^{\rm (HE)}(\alpha,\mu_1,\mu_2,x_i)$, using the definition in \eqref{DEFHE}\;
    Determine $r_{i+1}$ by \eqref{RiHE}, $v_{i+1}$ by \eqref{ViHE}\;
   }{
   Perform ME phase-type fit: given $r_i$ and $v_i$, determine $p,k,\mu$\;
   ${\mathscr L}^{({\rm Ph})} ( {\boldsymbol x}):={\mathscr L}^{({\rm Ph})} ( {\boldsymbol x})+{\mathscr L}^{\rm (ME)}(p,k,\mu,x_i)$, using the definition in \eqref{DEFME}\;
   Determine $r_{i+1}$ by \eqref{RiME}, $v_{i+1}$ by \eqref{ViME}\;
  }
  $i:=i+1$\;
 }
 \caption{Approximation algorithm: Phase-type fit}
 \label{algo}
\end{algorithm}}

\vspace{3mm}


{\small
\begin{algorithm}[H]
 \KwData{$(\beta_1,\ldots,\beta_n)$,  $(\sigma_1^2,\ldots,\sigma_n^2)$, $(x_1,\ldots,x_n)$.}
 \KwResult{$(r_1,\ldots,r_n)$,  $(v_1,\ldots,v_n),$ ${\mathscr L}^{({\rm W})} ( {\boldsymbol x})$.}
 Initialization: $i:=1$\;
 $r_1:=\beta_1$, $v_1:=\sigma_1^2$\;
  ${\mathscr L}^{({\rm W})} ( {\boldsymbol x}):=0$\;
 \While{$i < n$}{
   Perform Weibull fit: given $r_i$ and $v_i$, determine $\lambda,\alpha$\;
   ${\mathscr L}^{({\rm W})} ( {\boldsymbol x}):={\mathscr L}^{({\rm W})} ( {\boldsymbol x})+{\mathscr L}^{\rm (W)}(\alpha,\lambda,x_i)$, using the definition in \eqref{DEW}\;
    Determine $r_{i+1}$ by \eqref{RiW}, $v_{i+1}$ by \eqref{ViW}\;
  $i:=i+1$\;
 }
 \caption{Approximation algorithm: Weibull fit}
 \label{algo}
\end{algorithm}}

\vspace{3mm}

{\small 
\begin{algorithm}[H]
 \KwData{$(\beta_1,\ldots,\beta_n)$,  $(\sigma_1^2,\ldots,\sigma_n^2)$, $(x_1,\ldots,x_n)$.}
 \KwResult{$(r_1,\ldots,r_n)$,  $(v_1,\ldots,v_n),$ ${\mathscr L}^{({\rm LN})} ( {\boldsymbol x})$.}
 Initialization: $i:=1$\;
 $r_1:=\beta_1$, $v_1:=\sigma_1^2$\;
  ${\mathscr L}^{({\rm LN})} ( {\boldsymbol x}):=0$\;
 \While{$i < n$}{
   Perform Lognormal fit: given $r_i$ and $v_i$, determine $\mu,\tau^2$\;
   ${\mathscr L}^{({\rm LN})} ( {\boldsymbol x}):={\mathscr L}^{({\rm LN})} ( {\boldsymbol x})+{\mathscr L}^{\rm (LN)}(\mu,\tau^2,x_i)$, using the definition in \eqref{DEFLN}\;
    Determine $r_{i+1}$ by \eqref{RiLN}, $v_{i+1}$ by \eqref{ViLN}\;
  $i:=i+1$\;
 }
 \caption{Approximation algorithm: Lognormal fit}
 \label{algo}
\end{algorithm}}
\vspace{3mm}


==> Sections/preliminaries.tex <==
\section{Preliminaries}\label{PREL}
In this section we first present the phase-type fit (based on the first two moments, that is) as well as a few auxiliary results. Then two alternative fitting techniques are presented, also based on the first two moments, viz.\ the Weibull and Lognormal fits. In the last subsection we point out how the objective function ${\mathscr L}({\boldsymbol x})$ can be evaluated for each of the three fits. 
Throughout this paper, for any non-negative random variable $X$, we denote by $f_X(\cdot)$ its density, which we assume to exist.

\subsection{Phase-type fit}
A crucial idea in our approach is that non-negative random variables can be approximated by phase-type distributions. It is well known from the literature that they can do this arbitrarily accurately; see e.g.\ Asmussen \cite[Thm.\ III.4.2]{asmussen2003}. To obtain an accurate fit, however, the dimension of the underlying phase-type distribution can become large. This triggered the idea of phase-type approximations of relatively low dimension, chosen such that the approximating distribution has the same first two moments as the target distribution (the `two-moments fit'). In this low-dimensional approximation, the phase-type distributions used are mixtures of Erlang distributions and hyperexponential distributions. 
Due to the fact that phase-type distributions inherently lead to a Markovian system, explicit expressions for various queueing-related metrics are available, such as the idle and waiting time distributions (where in this context ‘explicit’ means in terms of eigenvalues/eigenvectors of an associated eigensystem).


The two-moments fit we will be applying is the one presented in Tijms \cite{tijms1986}, matching the first and second moment, or, equivalently, the mean and the squared coefficient of variation ({\sc scv}). The {\sc scv} of the random variable $X$ is defined as its variance ${\mathbb V}{\rm ar}\,X$ divided by the square of the mean ${\mathbb E}X$. As prescribed by the fit presented in \cite{tijms1986}, we choose to match a mixture of two Erlang distributions in case $X$ has an {\sc scv} smaller than 1, and a hyperexponential distribution in case of an {\sc scv} larger than  1. 
An attractive feature of this specific phase-type fit is that it is of relatively low dimension \bs{do we need to mention this again?}. 

\vb

We continue by reviewing a few (known) elementary properties of hyperexponential distributions and of mixtures of Erlang distributions, and proceed by computing for both distributions the quantities ${\mathbb E}(X-x)^+$ and ${\mathbb E}(x-X)^+$, which we need for our objective function.
\begin{itemize}
    \item[$\circ$]
    Supposing that $X$ is hyperexponential, with (positive) parameters $\alpha,\mu_1$ and $\mu_2$, denoted by $X\sim  {\rm HE}(\alpha,\mu_1,\mu_2)$, then the underlying density is
    \[f_X(x) = \alpha \,\mu_1e^{-\mu_1 x} + (1-\alpha) \,\mu_2e^{-\mu_2 x} .\]
It is readily verified that
\[{\mathbb E}\,X = \frac{\alpha}{\mu_1}+\frac{1-\alpha}{\mu_2},\:\:\:\:
{\mathbb V}{\rm ar}\,X =  \frac{\alpha}{\mu_1^2}+ \frac{1-\alpha}{\mu_2^2} + \alpha (1-\alpha) \Big(\frac{1}{\mu_1}-\frac{1}{\mu_2} \Big)^2.\] 
For $X\sim  {\rm HE} 
(\alpha,\mu_1,\mu_2)$ an elementary calculation reveals that
\begin{align} \label{eqn:excess-HE}
    {\mathbb E}(X-x)^+ & = \frac{\alpha}{\mu_1} e^{-\mu_1 x} + \frac{1-\alpha}{\mu_2}  e^{-\mu_2 x},
\end{align}
an expression that could have also been derived using the memoryless property of the exponential distribution.
 \item[$\circ$]
Supposing that $X$ is mixed Erlang, with parameters $p\in[0,1]$, $k\in{\mathbb N}$ and $\mu>0$, denoted by $X\sim {\rm ME}(p,k,\mu)$, then %\footnote{Please check!}
the underlying density is
\begin{equation}\label{MED}f_X(x) = p \,\frac{\mu^{k-1}x^{k-2}}{(k-2)!} e^{-\mu x}+ (1-p)\,\frac{\mu^kx^{k-1}}{(k-1)!} e^{-\mu x}.\end{equation}
It requires a few elementary integrations to check that
\[{\mathbb E}\,X = p\frac{k-1}{\mu}+(1-p)\frac{k}{\mu}=\frac{k-1}{\mu}+\frac{1-p}{\mu},\:\:\:\:
{\mathbb V}{\rm ar}\,X = \frac{k-p^2}{\mu^2} .\]
For $X\sim {\rm ME}(p,k,\mu)$ a lengthy calculation (given in Appendix \ref{APP}), shows that
 \begin{align}\notag
     {\mathbb E}(X-x)^+ & = \int_x^\infty f_X(y) (y-x)\,{\rm d}y \\& \notag= \int_x^\infty \bigg( p\frac{\mu^{k-1} y^{k-2}e^{-\mu y}}{(k-2)!}+ (1-p)\frac{\mu^{k} y^{k-1}e^{-\mu y}}{(k-1)!}\bigg) (y-x)\,{\rm d}y \\ \label{eqn:excess-ME}
     & = \frac{k-p-\mu x}{\mu (k-2)!}\Gamma(k-1, \mu x) + \frac{k-p}{\mu(k-1)!}(\mu x)^{k-1}e^{-\mu x};
     %\\
     %& = \frac{e^{-\mu x} (k-p-\mu x)}{\mu} \sum_{l=0}^{k-2} \frac{(\mu x)^l}{l!} + \frac{(k-p)}{\mu(k-1)!}(\mu x)^{k-1}e^{-\mu x} \\
     %& = 
    % & = \text{\bs{further reduction can be done}}
 \end{align}
here $\Gamma(k,t)$ denotes the incomplete Gamma integral $\int_t^\infty z^{k-1} e^{-z}\,{\rm d}z$ which can be called in any standard numerical software package. In the above calculation, various standard properties of the incomplete Gamma integral have been used. 
\end{itemize}

\subsection{Weibull fit}
Supposing that $X$ is Weibull, with positive parameters $\alpha$ and $\lambda$, denoted by  $X\sim {\rm W}(\lambda,\alpha)$, then the underlying density function is given by
\[f_X(x)= \alpha \lambda^\alpha x^{\alpha-1} e^{-(\lambda x)^\alpha}.%\:\:\:\:
%F_X(x) = 1 - e^{-(\lambda x)^\alpha}, \bs{I don't think we need cdf here}
\]
%respectively; we write $X\sim {\rm W}(\lambda,\alpha)$.
It is known that
\[{\mathbb E}\,X= \lambda^{-1} \Gamma(1+1/\alpha),\:\:\:{\mathbb V}{\rm ar}X = \lambda^{-2}\big(\Gamma(1+2/\alpha)-(\Gamma(1+1/\alpha))^2\big),\]
so that the corresponding squared coefficient of variation equals
\[\frac{\Gamma(1+2/\alpha)-(\Gamma(1+1/\alpha))^2}{(\Gamma(1+1/\alpha))^2},\]
which decreases from $\infty$ to $0$ as $\alpha$ increases from $0$ to $\infty$, so that for each value of the squared coefficient of variation there is a unique $\alpha$, and hence also a unique $\lambda$.

Also, applying integration by parts in the second equality, and the substitution $w=(\lambda y)^\alpha$ in the fourth, 
\begin{align}
  {\mathbb E}(X-x)^+ \notag & = \int_x^\infty f_X(y) (y-x)\,{\rm d}y = \int_x^\infty (1-F_X(y))\,{\rm d}y= \int_x^\infty e^{-(\lambda y)^\alpha}\,{\rm d}y\\\label{EW}&=    \frac{1}{\lambda\alpha}\int_{(\lambda x)^\alpha}^\infty w^{1/\alpha -1} e^{-w}\,{\rm d}w = {\frac{1}{\lambda\alpha} \Gamma(1/\alpha, (\lambda x)^\alpha) }.
\end{align}  
This can be further rewritten to
\begin{align}
  \notag
  \alpha \lambda^\alpha& \int_x^\infty y^\alpha e^{-(\lambda y)^\alpha}\,{\rm d}y - \alpha \lambda^\alpha x\int_x^\infty y^{\alpha-1} e^{-(\lambda y)^\alpha}\,{\rm d}y
  \\ \notag
  & = \int_{(\lambda x)^\alpha}^\infty \frac{w^{{1}/{\alpha}}e^{-w}}{\lambda}\,{\rm d}w- x\int_{(\lambda x)^\alpha}^\infty e^{-w}\,{\rm d}w = \frac{1}{\lambda} \Gamma(1+1/\alpha, (\lambda x)^\alpha) - x\,e^{-(\lambda x)^\alpha}.
\end{align}

\subsection{Lognormal fit}
Supposing that $X$ is Lognormal, with parameters $\mu \in (-\infty, +\infty)$ and $\tau>0$, denoted by $X\sim {\rm LN}(\mu,\tau^2)$, then the underlying density is 
\[ { f_X(x)=\frac{1}{ \sqrt{2\pi}\tau x} \exp\left(-\frac{(\log x-\mu)^2}{2\tau^2}\right).}\]
%in the sequel denoted by $X\sim {\rm LN}(\mu,\tau^2)$, where 
It can be verified that
\[{\mathbb E}\,X = e^{\mu+\tau^2/2},\:\:\:{\mathbb V}{\rm ar} X =(e^{\tau^2}-1) \,e^{2\mu+\tau^2}, \]
entailing that the corresponding squared coefficient of variation is $e^{\tau^2}-1$. The squared coefficient of variation increases from~$0$ to $\infty$ as $\tau^2$ increases from~$0$ to $\infty.$ Hence,   for each value of the squared coefficient of variation there is a unique $\tau^2$, and thus also a unique $\mu$.


Also, applying the transformation $w=\log y$ in the third equality, and isolating the square in the fourth,
\begin{align}\notag
  {\mathbb E}(X-x)^+ & = \int_x^\infty f_X(y) (y-x)\,{\rm d}y =  \int_x^\infty
  (y-x) \,\frac{1}{\sqrt{2\pi}\tau y} \exp\left(-\frac{(\log y-\mu)^2}{2\tau^2}\right)\,{\rm d}y\\\notag
  &=\int_{\log x}^\infty (e^w-x) \frac{1}{\sqrt{2\pi}\tau} \exp\left(-\frac{(w-\mu)^2}{2\tau^2}\right){\rm d}w \\\notag
 % &= \bs{\frac{1}{\tau\sqrt{2\pi}} \Bigg[ \int_{\log x}^\infty (e^{-\frac{(w-\mu )^2}{2\tau^2}}-\frac{x}{e^w} e^{-\frac{(w-\mu )^2}{2\tau^2}})e^w dw  \Bigg] }\\ \notag
  %& = \bs{ \frac{1}{\tau\sqrt{2\pi}} \int_{\log x}^\infty e^{-\frac{(w-\mu )^2}{2\tau^2}} (e^w -x) dw }\\ \notag
  %& = \bs{\frac{1}{\tau\sqrt{2\pi}} \Bigg((\int_{\log x}^\infty e^{-(\frac{w}{\sqrt{2}\tau}-\frac{\tau^2(\mu/\tau^2+1)}{\sqrt{2}} )^2 +\frac{\tau^2(m/\tau^2+1)^2}{2}-\frac{\mu^2}{2\tau^2}} dw - x\int_{\log x}^\infty \exp\left(-\frac{(w-\mu)^2}{2\tau^2}\right){\rm d}w \Bigg) } \\ \notag
 %& = \bs{\frac{1}{\tau\sqrt{2\pi}} \Bigg( \frac{\sqrt{\pi}}{\sqrt{2}}\tau e^{\frac{(\mu/\tau^2+1)s^2}{2}-\frac{\mu^2}{2\tau^2}}\int_{\frac{log(x)-\tau^2-\mu}{\tau\sqrt{2}}}^\infty \frac{2e^{-v^2}}{\sqrt{\pi}}dv -x\int_{\log x}^\infty \exp\left(-\frac{(w-\mu)^2} {2\tau^2}\right){\rm d}w\Bigg)}\\ \notag
 %&= \bs{\frac{1}{\tau\sqrt{2\pi}} \Bigg( \frac{\sqrt{\pi}}{\sqrt{2}}\tau e^{\frac{(\mu/\tau^2+1)s^2}{2}-\frac{\mu^2}{2\tau^2}}(1-erf(\frac{log(x)-\tau^2-\mu}{\tau\sqrt{2}})) -x\int_{\log x}^\infty \exp\left(-\frac{(w-\mu)^2} {2\tau^2}\right){\rm d}w\Bigg)}\\
   & = \frac{1}{\sqrt{2\pi}\tau}\left(e^{\mu+\tau^2/2}\int_{\log x}^\infty \exp\left(-\frac{(w-(\mu+\tau^2))^2}{2\tau^2}\right){\rm d}w - x\int_{\log x}^\infty \exp\left(-\frac{(w-\mu)^2}{2\tau^2}\right){\rm d}w 
  \right)\\
  &\notag = e^{\mu+\tau^2/2} \,{\mathbb P}({\rm N}(\mu+\tau^2,\tau^2)>\log x) - x \,{\mathbb P}({\rm N}(\mu,\tau^2)>\log x)\\
   &=e^{\mu+\tau^2/2} \Psi\left(\frac{\log x - \mu-\tau^2}{\tau}\right) - x \,\Psi\left(\frac{\log x-\mu}{\tau}\right),\label{ELN}
  \end{align}
  with $\Psi(x):=\int_x^\infty (\sqrt{2\pi})^{-1}\exp(-y^2/2)\,{\rm d}y$ denoting the standard Normal complementary distribution function, and $X\sim {\rm N}(\mu,\tau^2)$ denoting that $X$ is Normally distributed with mean $\mu$ and variance $\tau^2$. 


\subsection{Evaluation of objective function}\label{EOF}
When aiming at the computation of the objective function \eqref{OBJ}, a useful key identity is: for weights $A$ and $B$ and a constant $x\geqslant 0$,
\begin{equation*}
    A(X-x)1\{X\geqslant x\}+B(x-X)1\{X<x\}=(A+B)(X-x)1\{X\geqslant x\}+B(x-X),
\end{equation*}
so that
\begin{equation*}
      {\mathscr L} ( {\boldsymbol x})=  \sum_{j=1}^n 
      {\mathscr L}_j ( {x}_{j-1}),\:\:\:\:
      {\mathscr L}_j ( {x}):=
      {\mathbb E}\big(R_{j-1} - x\big)^+ + \omega\,{\mathbb E}\big(x - R_{j-1}\big)
\end{equation*}
We proceed by pointing out how one can compute $ {\mathscr L}_j ( {x})$ in case $R_{j-1}$ has a phase-type, Weibull or Lognormal distribution.
%In the phase-type case, we consecutively consider the cases that $R_{j-1}$ is hyperexponential and mixed Erlang.
\begin{itemize}
    \item[$\circ$] In the phase-type case, suppose that $R_{j-1}\sim  {\rm HE}(\alpha,\mu_1,\mu_2)$ for some $\alpha,\mu_1,\mu_2>0.$ Then, relying on \eqref{eqn:excess-HE},
\begin{equation}\label{DEFHE}
    {\mathscr L}_j ( {x})= \frac{\alpha}{\mu_1}(e^{-\mu_1 x} -\omega) + \frac{(1-\alpha)}{\mu_2}(e^{-\mu_2 x} -\omega) + \omega x =:{\mathscr L}^{\rm (HE)}(\alpha,\mu_1,\mu_2,x).
\end{equation}
Suppose that $R_{j-1}\sim {\rm ME}(p,k,\mu)$ for some $p\in[0,1]$, $k\in{\mathbb N}$ and $\mu>0$. Then, by \eqref{eqn:excess-ME},
\begin{align} %old version 
    \notag {\mathscr L}_j ( {x}) &=  \frac{k-p-\mu x}{\mu (k-2)!}\Gamma(k-1, \mu x) + \frac{k-p}{\mu(k-1)!}(\mu x)^{k-1}e^{-\mu x} + \omega \left(x- \frac{k-p}{\mu}\right)\\
    &=:{\mathscr L}^{\rm (ME)}(p,k,\mu,x).
\label{DEFME}
\end{align}
    \item[$\circ$] In the Weibull case, if $R_{j-1}\sim {\rm W}(\lambda,\alpha)$, then, by \eqref{EW},
\begin{align} %old version 
    {\mathscr L}_j ( {x}) &=  
 \frac{1}{\lambda} \Gamma(1+1/\alpha, (\lambda x)^\alpha) - x\,e^{-(\lambda x)^\alpha} +\omega x -\frac{\omega}{\lambda}\Gamma(1+1/\alpha)=:{\mathscr L}^{\rm (W)}(\alpha,\lambda,x).
\label{DEW}
\end{align}
    \item[$\circ$] In the Lognormal case, if $R_{j-1}\sim {\rm LN}(\mu,\tau^2)$, then, by \eqref{ELN},
\begin{align} %old version 
\notag
   {\mathscr L}_j ( {x}) &=  
   e^{\mu+\tau^2/2} \,\left(\Psi\left(\frac{\log x-\mu-\tau^2}{\tau}\right)-\omega\right) -  x\left(\Psi\left(\frac{\log x-\mu}{\tau}\right)-\omega\right)\\&=:{\mathscr L}^{\rm (LN)}(\mu,\tau^2,x).
\label{DEFLN}
\end{align}
\end{itemize}


==> tables/BWtable.tex <==
\begin{table}[h]
\begin{tabular}{llllll}
\toprule
\textbf{n} &\multicolumn{1}{l}{\textbf{\sc scv}} & \multicolumn{1}{l}{$\boldsymbol x $}                  & \multicolumn{1}{l}{\textbf{PTA}}   & \multicolumn{1}{l}{\textbf{EPTA}}       & \textbf{Lognormal}                  \\ \hline
%\multicolumn{6}{|l|}{Bailey-Welch}                                                                                                                                                    \\ \hline
\multirow{3}{*}{10 } &\multicolumn{1}{l}{0.6} & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{5.78} & \multicolumn{1}{l}{5.86} & \multicolumn{1}{l} {5.74} \\
&\multicolumn{1}{l}{1}   & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{7.04} & \multicolumn{1}{l}{6.91} & \multicolumn{1}{l} {6.56} \\ 
&\multicolumn{1}{l}{1.6} & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{7.93} & \multicolumn{1}{l}{7.95} & \multicolumn{1}{l} {7.46} \\
\cline{1-6}
\multirow{3}{*}{40 } &\multicolumn{1}{l}{0.6}   & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{40.68} & \multicolumn{1}{l}{39.81} & \multicolumn{1}{l} {39.25} \\ 
&\multicolumn{1}{l}{1} & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{50.43} & \multicolumn{1}{l}{49.15} & \multicolumn{1}{l} {47.79} \\ 
&\multicolumn{1}{l}{1.6} & \multicolumn{1}{l}{{[}0, 1, 1, 1...{]}} & \multicolumn{1}{l}{60.14} & \multicolumn{1}{l}{58.14} & \multicolumn{1}{l} {57.00} \\ 

\bottomrule
\end{tabular}
\caption{ Comparing results using classic Bailey-Welch interarrival times. }
\label{BWT}
\end{table}


==> tables/compare_log_weibul.tex <==
\begin{center}
    \begin{longtable}{lllrrrrrrr}%{|lllllllll|lll|}
 
%\begin{table}[]
%\begin{tabular}{llllllllllll}
\toprule
%\hline

\textbf{n} & \textbf{SCV}                  & $\boldsymbol x $  & \multicolumn{1}{l}{\textbf{PTA}} & \multicolumn{1}{l}{\textbf{EPTA}} & \multicolumn{1}{l}{\textbf{Lognormal}} & \multicolumn{1}{l}{\textbf{Weibull}} & \multicolumn{1}{l}{\textbf{$\Delta_{PTA}$}} & \multicolumn{1}{l}{\textbf{$\Delta_{Lognormal}$}} & \multicolumn{1}{l}{\textbf{$\Delta_{Weibull}$}} \\ 
\cline{1-10}
\multirow{27}{*}{10} & \multirow{9}{*}{\textbf{0.5}} & 1.1 & 3.95                     & 3.94                     & 3.83                          & 3.98                        & 0.43                                     & 2.83                                & 1.02                               \\
                &     & 1.2 & 3.72                     & 3.72                     & 3.65                          & 3.74                        & 0.06                                     & 1.81                                & 0.40                               \\
                &     & 1.3 & 3.70                     & 3.70                     & 3.70                          & 3.69                        & 0.06                                     & 0.09                                & 0.40                               \\
                 &    & 1.4 & 3.84                     & 3.84                     & 3.87                          & 3.81                        & 0.08                                     & 0.72                                & 0.70                               \\
                &     & 1.5 & 4.11                     & 4.10                     & 4.17                          & 4.08                        & 0.17                                     & 1.53                                & 0.56                               \\
                &     & 1.6 & 4.46                     & 4.45                     & 4.54                          & 4.42                        & 0.19                                     & 1.91                                & 0.67                               \\
                &     & 1.7 & 4.88                     & 4.87                     & 4.97                          & 4.84                        & 0.17                                     & 2.03                                & 0.54                               \\
                 &    & 1.8 & 5.34                     & 5.33                     & 5.43                          & 5.30                        & 0.13                                     & 1.82                                & 0.59                               \\
                 &    & 1.9 & 5.83                     & 5.82                     & 5.92                          & 5.79                        & 0.10                                     & 1.58                                & 0.59                               \\ \cline{2-10}%\hline
&\multirow{9}{*}{\textbf{1}}   & 1.1 & 5.70                     & 5.65                     & 5.29                          & 5.71                        & 0.86                                     & 6.36                                & 1.07                               \\
              &       & 1.2 & 5.40                     & 5.37                     & 5.09                          & 5.40                        & 0.55                                     & 5.22                                & 0.49                               \\
                &     & 1.3 & 5.28                     & 5.26                     & 5.06                          & 5.28                        & 0.32                                     & 3.83                                & 0.40                               \\
                  &   & 1.4 & 5.29                     & 5.28                     & 5.15                          & 5.29                        & 0.17                                     & 2.45                                & 0.20                               \\
                 &    & 1.5 & 5.41                     & 5.40                     & 5.33                          & 5.41                        & 0.08                                     & 1.25                                & 0.08                               \\
                  &   & 1.6 & 5.62                     & 5.62                     & 5.60                          & 5.61                        & 0.04                                     & 0.30                                & 0.10                               \\
                 &    & 1.7 & 5.90                     & 5.90                     & 5.93                          & 5.91                        & 0.01                                     & 0.39                                & 0.11                               \\
                  &   & 1.8 & 6.25                     & 6.25                     & 6.30                          & 6.26                        & 0.00                                     & 0.88                                & 0.16                               \\
                  &   & 1.9 & 6.63                     & 6.63                     & 6.71                          & 6.63                        & 0.00                                     & 1.18                                & 0.09                               \\ \cline{2-10}
& \multirow{9}{*}{\textbf{1.5}} & 1.1 & 6.72                     & 6.55                     & 6.26                          & 6.87                        & 2.52                                     & 4.42                                & 4.84                               \\
                 &    & 1.2 & 6.47                     & 6.27                     & 6.05                          & 6.62                        & 3.15                                     & 3.48                                & 5.63                               \\
                &     & 1.3 & 6.35                     & 6.15                     & 6.03                          & 6.45                        & 3.36                                     & 1.96                                & 5.01                               \\
                 &    & 1.4 & 6.35                     & 6.16                     & 6.04                          & 6.41                        & 3.19                                     & 1.86                                & 4.12                               \\
                 &    & 1.5 & 6.44                     & 6.27                     & 6.20                          & 6.48                        & 2.79                                     & 1.18                                & 3.32                               \\
                 &    & 1.6 & 6.62                     & 6.47                     & 6.43                          & 6.64                        & 2.28                                     & 0.65                                & 2.63                               \\
                 &    & 1.7 & 6.85                     & 6.73                     & 6.74                          & 6.85                        & 1.78                                     & 0.03                                & 1.75                               \\
                &     & 1.8 & 7.14                     & 7.05                     & 7.03                          & 7.12                        & 1.33                                     & 0.23                                & 1.02                               \\
                  &   & 1.9 & 7.48                     & 7.41                     & 7.40                          & 7.45                        & 0.95                                     & 0.13                                & 0.50                               \\ \cline{1-10}
\multirow{27}{*}{40} & \multirow{9}{*}{\textbf{0.5}} & 1.1 & 23.53                    & 23.66                    & 23.21                         & 23.64                       & 0.54                                     & 1.88                                & 0.06                               \\
                &     & 1.2 & 18.14                    & 18.16                    & 18.23                         & 18.04                       & 0.12                                     & 0.38                                & 0.67                               \\
                &     & 1.3 & 16.06                    & 15.97                    & 16.32                         & 15.90                       & 0.57                                     & 2.22                                & 0.43                               \\
                 &    & 1.4 & 15.80                    & 15.69                    & 16.17                         & 15.65                       & 0.67                                     & 3.02                                & 0.26                               \\
                &     & 1.5 & 16.52                    & 16.43                    & 16.90                         & 16.35                       & 0.54                                     & 2.89                                & 0.47                               \\
                &     & 1.6 & 17.79                    & 17.72                    & 18.19                         & 17.64                       & 0.39                                     & 2.65                                & 0.45                               \\
               &      & 1.7 & 19.41                    & 19.35                    & 19.82                         & 19.25                       & 0.27                                     & 2.42                                & 0.53                               \\
                 &    & 1.8 & 21.24                    & 21.20                    & 21.62                         & 21.09                       & 0.18                                     & 2.02                                & 0.50                               \\
                &     & 1.9 & 23.21                    & 23.18                    & 23.59                         & 23.06                       & 0.12                                     & 1.77                                & 0.52                               \\ \cline{2-10}
& \multirow{9}{*}{\textbf{1}}   & 1.1 & 36.72                    & 36.28                    & 35.07                         & 36.80                       & 1.21                                     & 3.33                                & 1.44                               \\
              &       & 1.2 & 29.61                    & 29.48                    & 28.77                         & 29.53                       & 0.45                                     & 2.41                                & 0.20                               \\
                &     & 1.3 & 25.53                    & 25.51                    & 25.22                         & 25.45                       & 0.11                                     & 1.11                                & 0.20                               \\
                 &    & 1.4 & 23.52                    & 23.52                    & 23.61                         & 23.52                       & 0.01                                     & 0.37                                & 0.02                               \\
               &      & 1.5 & 22.86                    & 22.86                    & 23.13                         & 22.83                       & 0.00                                     & 1.17                                & 0.11                               \\
                 &    & 1.6 & 23.07                    & 23.07                    & 23.49                         & 23.08                       & 0.00                                     & 1.83                                & 0.06                               \\
               &      & 1.7 & 23.85                    & 23.85                    & 24.42                         & 23.84                       & 0.00                                     & 2.36                                & 0.06                               \\
            &         & 1.8 & 25.03                    & 25.03                    & 25.57                         & 25.04                       & 0.00                                     & 2.19                                & 0.05                               \\
                &     & 1.9 & 26.47                    & 26.47                    & 27.05                         & 26.48                       & 0.00                                     & 2.16                                & 0.02                               \\ \cline{2-10}
 & \multirow{9}{*}{\textbf{1.5}} & 1.1 & 45.83                    & 43.53                    & 43.48                         & 46.55                       & 5.29                                     & 0.10                                & 6.95                               \\
            &         & 1.2 & 38.39                    & 36.15                    & 36.73                         & 38.65                       & 6.20                                     & 1.63                                & 6.92                               \\
                 &    & 1.3 & 33.57                    & 31.82                    & 32.44                         & 33.61                       & 5.49                                     & 1.92                                & 5.60                               \\
                  &   & 1.4 & 30.68                    & 29.49                    & 30.00                         & 30.70                       & 4.03                                     & 1.72                                & 4.10                               \\
                 &    & 1.5 & 29.17                    & 28.43                    & 28.75                         & 29.07                       & 2.61                                     & 1.14                                & 2.25                               \\
                &     & 1.6 & 28.63                    & 28.20                    & 28.47                         & 28.52                       & 1.53                                     & 0.97                                & 1.14                               \\
                 &    & 1.7 & 28.78                    & 28.54                    & 28.90                         & 28.58                       & 0.81                                     & 1.24                                & 0.14                               \\
                 &    & 1.8 & 29.41                    & 29.31                    & 29.52                         & 29.25                       & 0.37                                     & 0.74                                & 0.18                               \\
                 &    & 1.9 & 30.41                    & 30.38                    & 30.58                         & 30.23                       & 0.11                                     & 0.67                                & 0.48                               \\ 
\bottomrule
%\end{tabular}
\caption{ Fixed interarrival times and loss in case of PTA {\it (paper-1)}, simulated Lognormal and Weibull service times compared with our approach.}
\label{t2long}
\end{longtable}

\end{center}

==> tables/execution_time.tex <==

\begin{table}[h]
\begin{tabular}{lllllllll}
\toprule
n  & $\mathscr{L}(x_{\mathrm{Eq}})$ & ${\mathscr L}^{Ph}({ x}_{\rm Eq})$ & ${\mathscr L}^{W}({ x}_{\rm Eq})$ & ${\mathscr L}^{LN}({ x}_{\rm Eq})$ & $x^*$   & $x^*_{Ph}$ & $x^*_{W}$ & $x^*_{LN}$\\
\midrule
5  & 0.0014    & 4.8757e-05  & 0.0025 & 3.6105e-04 & 0.0302  & 5.7311e-04  & 0.1658  & 0.0304 \\
10 & 0.0038    & 9.5860e-05  & 0.0059 & 8.0760e-04 & 0.2090  & 5.3298e-04   & 0.9765 &0.1009\\
15 & 0.0156    & 1.4417e-04  & 0.0084 & 0.0013 & 2.0307  & 6.9113e-04  & 1.9912 & 0.2217 \\
20 & 0.0255    & 1.9334e-04  & 0.0123 & 0.0017 & 5.2713  & 7.3734e-04  &2.9342 & 0.4306\\
25 & 0.0465    & 2.4748e-04  & 0.0154 & 0.0022 & 11.7156 & 7.5564e-04  & 4.1027 & 0.6698\\
30 & 0.0538    & 2.9150e-04  & 0.0185 & 0.0026 & 22.3102 & 8.4637e-04  & 7.3928 & 0.9598\\
35 & 0.0841    & 3.4007e-04  & 0.0218 & 0.0031 & 34.4167 & 9.2662e-04  & 11.9174& 1.3100\\
40 & 0.1201    & 3.8893e-04  & 0.0250 & 0.0035 & 52.6915 & 0.0010  & 13.9645 & 1.8870\\
\bottomrule
\end{tabular}
\caption{\label{time1} {\sc scv}=0.4}
\end{table} 

%(SCV=0.7)
\begin{table}[h]
\begin{tabular}{lllllllll}
\toprule
n  & $\mathscr{L}(x_{\mathrm{Eq}})$ & ${\mathscr L}^{Ph}({ x}_{\rm Eq})$ & ${\mathscr L}^{W}({ x}_{\rm Eq})$ & ${\mathscr L}^{LN}({ x}_{\rm Eq})$ & $x^*$   & $x^*_{Ph}$ & $x^*_{W}$ & $x^*_{LN}$ \\
\midrule
5  & 0.0010    & 5.8776e-05  & 0.0022 & 3.7257e-04 & 0.0237  & 4.4368e-04  & 0.1719  &0.0314\\
10 & 0.0015    & 1.2145e-04  & 0.0048 & 8.4652e-04 & 0.1156  & 5.4671e-04  & 0.9784 & 0.1102\\
15 & 0.0028    & 1.9854e-04  & 0.0077 & 0.0013 & 0.4207  & 6.1211e-04  & 1.6572 & 0.2720\\
20 & 0.0110    & 2.4915e-04  & 0.0111 & 0.0017 & 2.4006  & 7.6458e-04  & 3.8857 & 0.4410\\
25 & 0.0206    & 3.2258e-04  & 0.0136 & 0.0022 & 6.4486  & 8.7434e-04  & 4.7512 & 0.6737\\
30 & 0.0311    & 3.7965e-04  & 0.0166 & 0.0027 & 10.6372 & 0.0010  & 9.4110 & 1.0675\\
35 & 0.0417    & 4.4185e-04  & 0.0197 & 0.0031 & 17.7460 & 0.0011  & 14.1549 & 1.4810\\
40 & 0.0544    & 5.0984e-04  & 0.0230 & 0.0036 & 28.5703 & 0.0012 & 17.6238 & 1.9104\\
\bottomrule
\end{tabular}
\caption{\label{time2} {\sc scv}=0.7}
\end{table} 


%(SCV=1)
\begin{table}[h]
\begin{tabular}{lllllllll}
\toprule
n  & $\mathscr{L}(x_{\mathrm{Eq}})$ & ${\mathscr L}^{Ph}({ x}_{\rm Eq})$ & ${\mathscr L}^{W}({ x}_{\rm Eq})$ & ${\mathscr L}^{LN}({ x}_{\rm Eq})$ & $x^*$   & $x^*_{Ph}$ & $x^*_{W}$ & $x^*_{LN}$ \\
\midrule
5  & 0.0011  & 6.8888e-05  & 0.0019 & 3.6467e-04 & 0.0261  & 4.2792e-04 & 0.2081 & 0.0304 \\
10 & 0.0024  & 1.0925e-04  & 0.0048 & 8.3198e-04 & 0.1358  & 5.3788e-04 & 0.8250 & 0.1085\\
15 & 0.0033  & 1.7345e-04  & 0.0077 & 0.0013 & 0.4244  & 6.4661e-04 & 2.1580 & 0.2632\\
20 & 0.0134  & 2.3837e-04  & 0.0105 & 0.0018 & 2.7786  & 7.2551e-04 & 4.1389 & 0.4671\\
25 & 0.0264  & 3.0275e-04  & 0.0134 & 0.0022 & 6.7190  & 9.3613e-04 & 6.2367 & 0.7479\\
30 & 0.0392  & 3.6655e-04  & 0.0166 & 0.0027 & 12.2910 & 0.0010 & 9.2407 & 1.0697\\
35 & 0.0602  & 4.3190e-04  & 0.0192 & 0.0031 & 20.4043 & 0.0011 & 11.9491 & 1.4453\\
40 & 0.0707  & 4.9448e-04  & 0.0233 & 0.0036 & 28.3632 & 0.0012 & 15.4659 & 1.8831\\
\bottomrule
\end{tabular}
\caption{\label{time3} {\sc scv}=1}
\end{table} 


%(SCV=1.3)
\begin{table}[h]
\begin{tabular}{lllllllll}
\toprule
n  & $\mathscr{L}(x_{\mathrm{Eq}})$ & ${\mathscr L}^{Ph}({ x}_{\rm Eq})$ & ${\mathscr L}^{W}({ x}_{\rm Eq})$ & ${\mathscr L}^{LN}({ x}_{\rm Eq})$ & $x^*$   & $x^*_{Ph}$ & $x^*_{W}$ & $x^*_{LN}$ \\
\midrule
5  & 8.8299e-04 & 2.3547e-06  & 0.0026 & 3.6341e-04 & 0.0293  & 3.8048e-04 & 0.3094 & 0.0304\\
10 & 0.0015     & 2.9641e-06  & 0.0056 & 0.0012 & 0.1379  & 4.0399e-04 & 0.9438 & 0.1170\\
15 & 0.0032     & 3.1870e-06  & 0.0087 & 0.0014 & 0.4821  & 3.9733e-04 & 3.2037 & 0.2620 \\
20 & 0.0145     & 3.3842e-06  & 0.0115 & 0.0017 & 2.7294  & 4.4655e-04 & 4.9744 & 0.4657\\
25 & 0.0309     & 3.7135e-06  & 0.0147 & 0.0022 & 7.7266  & 4.4074e-04 & 7.3962 & 0.7267\\
30 & 0.0358     & 4.3253e-06  & 0.0181 & 0.0027 & 12.8194 & 4.4495e-04 & 10.0555 & 1.0569\\
35 & 0.0405     & 4.6143e-06  & 0.0214 & 0.0031 & 24.3923 & 4.4828e-04 & 13.8248 & 1.4702\\
40 & 0.0551     & 4.9959e-06  & 0.0258 & 0.0035 & 37.2561 & 5.3670e-04 & 22.0529 & 1.8729\\
\bottomrule
\end{tabular}
\caption{\label{time4} {\sc scv}=1.3}
\end{table} 


==> tables/optimised.tex <==
\begin{table}[]
\begin{tabular}{lllll}
\toprule
\textbf{n} & \textbf{SCV } & \textbf{PTA}              & \textbf{EPTA}              & \textbf{$\Delta$}            \\
\cline{1-5}
 \multirow{6}{*}{10 }& \textbf{0.6}        & \multicolumn{1}{c}{3.97} & \multicolumn{1}{c}{3.98} & \multicolumn{1}{c}{0.19} \\
& \textbf{0.8}        & \multicolumn{1}{c}{4.60} & \multicolumn{1}{c}{4.61} & \multicolumn{1}{c}{0.11} \\
& \textbf{1}          & \multicolumn{1}{c}{5.15} & \multicolumn{1}{c}{5.14} & \multicolumn{1}{c}{0.16} \\
& \textbf{1.2}        & \multicolumn{1}{c}{5.60} & \multicolumn{1}{c}{5.54} & \multicolumn{1}{c}{1.01} \\
& \textbf{1.4}        & \multicolumn{1}{c}{6.01} & \multicolumn{1}{c}{5.86} & \multicolumn{1}{c}{2.41} \\
& \textbf{1.6}        & \multicolumn{1}{c}{6.37} & \multicolumn{1}{c}{6.12} & \multicolumn{1}{c}{3.86} \\ \cline{1-5}
 \multirow{6}{*}{40 }& \textbf{0.4}        & 13.80                   & 13.74                    & 0.45                     \\
& \textbf{0.6}        & 17.11                    & 17.04                    & 0.42                     \\
& \textbf{0.8}        & 19.96                    & 19.94                    & 0.09                     \\
& \textbf{1}          & 22.57                    & 22.57                    & 0.01                     \\
& \textbf{1.2}        & 24.95                    & 24.87                    & 0.31                     \\
& \textbf{1.4}        & 27.14                    & 26.89                    & 0.89   \\ 
\bottomrule
\end{tabular}
\caption{\label{t1} Percentage difference changing with increasing squared coefficient of variation (scv).}
\end{table}

==> tables/tables_old.tex <==

\begin{table}[h]
\begin{tabular}{ll|ll|ll|ll}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{\sc scv}}} & \multicolumn{1}{l}{\multirow{2}{*}{$\mathbf{\it y}$}} & \multicolumn{2}{c}{\textbf{Phase-type}} & \multicolumn{2}{c}{\textbf{Weibull}}    & \multicolumn{2}{c}{\textbf{Lognormal}}            \\ \cline{3-8} 
\multicolumn{2}{l}{}                                              & ${\mathscr L}^{(\rm Ph)}({\boldsymbol x}_{\rm Eq}(y))$   & ${\mathscr L}({\boldsymbol x}_{\rm Eq}(y))$   & ${\mathscr L}^{(\rm W)}({\boldsymbol x}_{\rm Eq}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm Eq}(y))$ & ${\mathscr L}^{(\rm LN)}({\boldsymbol x}_{\rm Eq}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm Eq}(y))$ \\ \hline
\multirow{3}{*}{0.4}                     & 1.2                    & 17.15        & 17.13           & 17.10        & 17.04           & 17.00         & 17.40         \\
                                         & 1.5                           & 13.95 & 14.02           & 13.76        & 13.83           & 14.46         & 14.53         \\
                                         & 1.8                    & 17.63        & 17.66           & 17.46        & 17.49           & 18.07         & 18.11                 \\ \hline
\multirow{3}{*}{0.7}                     & 1.2                    & 26.57        & 26.43           & 26.59        & 26.53           & 24.55         & 26.22               \\
                                         & 1.5                    & 18.50        & 18.55           & 18.56        & 18.59           & 19.08         & 19.23              \\
                                         & 1.8                    & 20.13        & 20.17           & 20.16        & 20.18           & 20.87         & 20.93                \\ \hline
\multirow{3}{*}{1}                       & 1.2                    & 34.37        & 34.53           & 34.24        & 34.61           & 30.13         & 33.49          \\
                                         & 1.5                    & 23.39        & 23.40           & 23.41        & 23.41           & 23.33         & 23.80               \\
                                         & 1.8                    & 23.19        & 23.19           & 23.19        & 23.19           & 23.79         & 23.91             \\ \hline
\multirow{3}{*}{1.3}                     & 1.2   &    39.83                      & 41.26        &  40.59      & 41.63         & 34.54       & 39.62               \\
                                         & 1.5                            & 27.78  & 28.14       & 28.04      & 28.10         & 27.03       & 28.08        \\
                                         & 1.8                    & 26.43        & 26.45         & 26.31      & 26.30         & 26.62       & 26.88          \\ \bottomrule
\end{tabular}
\caption{\label{equi} Performance assessment for equidistant schedules.}
\end{table}



\begin{table}[h]
{\sciptsize
\begin{tabular}{l|ll|ll|ll}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{\sc scv}}} & \multicolumn{2}{c}{\textbf{Phase-type}} & \multicolumn{2}{c}{\textbf{Weibull}}    & \multicolumn{2}{c}{\textbf{Lognormal}}            \\ \cline{2-7} 
\multicolumn{1}{l}{} & ${\mathscr L}^{(\rm Ph)}({\boldsymbol x}_{\rm BW}(y))$      & ${\mathscr L}({\boldsymbol x}_{\rm BW}(y))$    &${\mathscr L}^{(\rm W)}({\boldsymbol x}_{\rm BW}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm BW}(y))$ & ${\mathscr L}^{(\rm LN)}({\boldsymbol x}_{\rm BW}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm BW}(y))$\\ \hline
0.4 & 18.78 & 18.74  & 18.77 & 18.70 & 18.47 & 18.90 \\
0.7 & 28.27 & 28.11 & 28.28 & 28.21 & 25.93 & 27.74 \\
1   & 35.99 & 36.17 & 35.85 & 36.25 & 31.39 & 34.97 \\
1.3 & 41.33 & 42.81 & 42.12 & 43.21 & 35.70 & 41.06 
 \\ \bottomrule
\end{tabular}
\caption{\label{baileyW} Performance assessment for Bailey-Welch schedules, $y=1.2$.}
}
\end{table}

\begin{table}[h]
{\scriptsize
\begin{tabular}{l|lll|lll|lll}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{\sc scv}}} & \multicolumn{3}{c}{\textbf{Phase-type}} & \multicolumn{3}{c}{\textbf{Weibull}}    & \multicolumn{3}{c}{\textbf{Lognormal}}            \\ \cline{2-10} 
\multicolumn{1}{l}{} & ${\mathscr L}^{(\rm Ph)}({\boldsymbol x}_{\rm BW}(y))$      & ${\mathscr L}({\boldsymbol x}_{\rm BW}(y))$  & $\Delta$  &${\mathscr L}^{(\rm W)}({\boldsymbol x}_{\rm BW}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm BW}(y))$ & $\Delta$& ${\mathscr L}^{(\rm LN)}({\boldsymbol x}_{\rm BW}(y))$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}_{\rm BW}(y))$& $\Delta$ \\ \hline
0.4 & 18.78 & 18.74 &0.21 & 18.77 & 18.70 & 0.37& 18.47 & 18.90 & 2.33 \\
0.7 & 28.27 & 28.11 & 0.59& 28.28 & 28.21 &0.24 & 25.93 & 27.74 & 6.97 \\
1   & 35.99 & 36.17 & 0.49& 35.85 & 36.25 &1.11 & 31.39 & 34.97 & 11.38 \\
1.3 & 41.33 & 42.81 & 3.46 & 42.12 & 43.21 &2.59 & 35.70 & 41.06 & 14.99
 \\ \bottomrule
\end{tabular}
\caption{\label{baileyW} Performance assessment for Bailey-Welch schedules, $y=1.2$.}
}
\end{table}


\begin{table}[h]
{\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llll|llll|llll}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{\sc scv}}} & \multicolumn{4}{c}{\textbf{Phase-type}} & \multicolumn{3}{c}{\textbf{Weibull}}    & \multicolumn{3}{c}{\textbf{Lognormal}}            \\ \cline{2-10} 
\multicolumn{1}{l}{}                                   &  ${\mathscr L}^{(\rm Ph)}({\boldsymbol x}^\star _{\rm Ph})$  &${\mathscr L}({\boldsymbol x}^\star )$    & ${\mathscr L}({\boldsymbol x}^\star _{\rm Ph})$    & ${\mathscr L}^{(\rm W)}({\boldsymbol x}^\star _{\rm W})$ &  ${\mathscr L}_{\rm sim}({\boldsymbol x}^\star _{\rm W})$ & ${\mathscr L}_{\rm sim}({\boldsymbol x}^\star _{\rm Ph})$ & ${\mathscr L}^{(\rm LN)}({\boldsymbol x}^\star _{\rm LN})$ & ${\mathscr L}_{\rm sim}(x^\star _{\rm LN})$ & ${\mathscr L}_{\rm sim}(x^\star _{\rm Ph})$ \\ \hline 
0.4 & 13.52 & 13.59 & 13.61 &13.34 & 13.65 & 13.47 & 13.97 & 13.66 & 14.14 \\
0.7 & 18.31 & 18.37 & 18.40 & 18.36 & 18.44 &18.47 &18.86 & 18.47 & 19.12\\
1  & 22.45&22.45 & 22.53& 22.45& 22.55 & 22.55& 22.72& 22.61 & 23.12\\
1.3  & 26.03& 26.09 & 26.21 & 25.97& 26.20& 26.28& 25.96 & 26.30 & 26.52 \\
\bottomrule
\end{tabular}
\caption{\label{optimSched} Performance assessment for optimized schedules.}
}
}

\end{table}




\begin{table}[h]
\begin{tabular}{c|lcll|lll|lll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textrm{scenario}}}  & \multicolumn{4}{c}{\textbf{Phase-type}} & \multicolumn{3}{c}{\textbf{Weibull}}    & \multicolumn{3}{c}{\textbf{Lognormal}}            \\ \cline{2-11} 
\multicolumn{1}{c}{}                                              & ${\mathscr L}$ &time   & ${\mathscr L}^{(\rm Ph)}$  &time   & ${\mathscr L}^{(\rm W)}$  &time  & ${\mathscr L}_{\rm sim}$ & ${\mathscr L}^{(\rm LN)}$ &time & ${\mathscr L}_{\rm sim}$ \\ \hline
A & 22.69 & 0.15 & 22.15 & $4.7\cdot 10^{-4}$& 22.38 & $2.1\cdot 10^{-2}$  & 22.47 & 21.95 & $3.7\cdot 10^{-3}$ & 24.24 \\
B & 24.05 & 0.14 & 24.35 &$3.0\cdot 10^{-4}$ & 24.28 & $2.2\cdot 10^{-2}$ & 24.26 & 24.54 & $3.5\cdot 10^{-3}$ & 26.11 \\
C & 22.93 & 0.12 & 22.78 & $2.8\cdot 10^{-4}$& 22.88 & $2.2\cdot 10^{-2}$ & 22.93 & 22.70 & $3.6\cdot 10^{-3}$ & 24.85 \\
D & 23.86 & 0.19 & 23.89 & $2.3\cdot 10^{-4}$ & 23.86 & $2.4\cdot 10^{-2}$ & 23.76 & 23.90 & $4.1\cdot 10^{-3}$ & 25.77 \\
E & 23.14 & 0.19 & 23.07 &$2.5\cdot 10^{-4}$ & 23.12 &  $2.5\cdot 10^{-2}$ & 23.11 & 23.02 & $3.9\cdot 10^{-3}$ & 25.52 \\
F & 23.66 & 0.13 & 23.68 & $2.8\cdot 10^{-4}$ & 23.67 & $2.5\cdot 10^{-2}$ & 23.57 & 23.63 & $3.8\cdot 10^{-3}$ & 25.01
  \\ \bottomrule
\end{tabular}
\caption{\label{heterogeneous} Performance assessment for heterogeneous scenarios.  For all the loss functions in this table the schedule ${\boldsymbol x}_{\rm Eq}(y)$ has been used, with $y=1.5$. Execution times are in seconds.}
\end{table}


\begin{table}[h]
{\scriptsize
\begin{tabular}{c|lcll|lll|lll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textrm{scenario}}}  & \multicolumn{4}{c}{\textbf{Phase-type}} & \multicolumn{3}{c}{\textbf{Weibull}}    & \multicolumn{3}{c}{\textbf{Lognormal}}            \\ \cline{2-11} 
\multicolumn{1}{c}{}                                              & ${\mathscr L}({\boldsymbol x}^\star)$ &time   & ${\mathscr L}^{(\rm Ph)}({\boldsymbol x}^\star _{\rm Ph})$  &time   & ${\mathscr L}^{(\rm W)}(x^\star _{\rm W})$  &time  & ${\mathscr L}_{\rm sim}({\boldsymbol x}^\star _{\rm W})$ & ${\mathscr L}^{(\rm LN)}(x^\star _{\rm LN})$ &time & ${\mathscr L}_{\rm sim}({\boldsymbol x}^\star _{\rm LN})$ \\ \hline
A & 21.97 & 44 & 21.84 & 0.0488 & 21.93 & 19.47  & 22.03& 21.89 & 2.14 & 24.61 \\
B & 22.56 & 49 & 22.55 &0.0125 &22.45 & 24.57 & 22.58 & 24.54& 2.46 & 24.37\\
C & 22.07 & 50 & 21.74 &0.0173 & 21.99 & 19.95 & 23.13 & 22.12 & 2.37 & 23.63 \\
D & 22.60 & 53 & 22.79   & 0.0165 & 22.50 & 22.62 & 22.60 & 23.08 & 2.49 & 23.78 \\
E & 22.20 & 44 & 22.12 &0.0116 & 22.56 &  17.96 & 22.60 & 22.97 & 2.38 & 24.07 \\
F & 22.61 & 36 & 22.61 & 0.0111 & 22.12 &17.46 & 21.08 &22.39 & 2.60 & 24.14
  \\ \bottomrule
\end{tabular}
\caption{\label{het_opt} Performance assessment for heterogeneous scenarios with optimized interarrival times. Execution times are in seconds.}
}
\end{table}





\begin{table}[h]
{\scriptsize
\begin{tabular}{c|lclll|llll|llll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textrm{scenario}}}  & \multicolumn{5}{c}{\textbf{Phase-type}} & \multicolumn{4}{c}{\textbf{Weibull}}    & \multicolumn{4}{c}{\textbf{Lognormal}}            \\ \cline{2-14} 
\multicolumn{1}{c}{}                                              & ${\mathscr L}$ &time   & ${\mathscr L}^{(\rm Ph)}$ &time   & $\Delta^{\rm Ph}$ & ${\mathscr L}^{(\rm W)}$  &time  & ${\mathscr L}_{\rm sim}$ & $\Delta^{\rm Ph}_{\rm W}$ & ${\mathscr L}^{(\rm LN)}$ &time & ${\mathscr L}_{\rm sim}$  & $\Delta^{\rm Ph}_{\rm LN}$\\ \hline
A & 22.69 & 0.15 & 22.40 & $4.7\cdot 10^{-4}$& 1.30 &22.64 & $2.1\cdot 10^{-2}$  & 22.70 & 1.32 & 22.17 & $3.7\cdot 10^{-3}$ & 22.88 & 2.10\\
B & 24.05 & 0.14 & 24.07 &$3.0\cdot 10^{-4}$ & 0.06 &24.00 & $2.2\cdot 10^{-2}$ & 23.99 & 0.33 & 24.30 & $3.5\cdot 10^{-3}$ & 24.48 & 1.67\\
C & 22.93 & 0.12 & 22.78 & $2.8\cdot 10^{-4}$&0.66 &22.88 & $2.2\cdot 10^{-2}$ & 22.90 &0.53 & 22.70 & $3.6\cdot 10^{-3}$ & 23.22 & 1.90\\
D & 23.86 & 0.19 & 23.89 & $2.3\cdot 10^{-4}$ & 0.16&23.86 & $2.4\cdot 10^{-2}$ & 23.78 & 0.48& 23.90 & $4.1\cdot 10^{-3}$ & 24.22 & 1.34\\
E & 23.14 & 0.19 & 23.07 &$2.5\cdot 10^{-4}$ & 0.30 & 23.12 &  $2.5\cdot 10^{-2}$ & 23.08 & 0.02& 23.02 & $3.9\cdot 10^{-3}$ & 23.45 & 1.60\\
F & 23.66 & 0.13 & 23.68 & $2.8\cdot 10^{-4}$ & 0.08 &23.67 & $2.5\cdot 10^{-2}$ & 23.59 & 0.40 & 23.63 & $3.8\cdot 10^{-3}$ & 23.99 & 1.28
  \\ \bottomrule
\end{tabular}
\caption{\label{heterogeneous} Performance assessment for heterogeneous scenarios.  For all the loss functions in this table the schedule ${\boldsymbol x}_{\rm Eq}(y)$ has been used, with $y=1.5$. Execution times are in seconds.}
}
\end{table}
